In-orbit performance of HE onboard Insight-HXMT in the first 5 years

Purpose: The High-Energy X-ray telescope (HE), one of the three main payloads of the \textit{Insight}-HXMT mission, is composed of eighteen NaI(Tl)/CsI(Na) phoswich detectors, where NaI(Tl) serves as the primary detector covering 20--250\,keV, and CsI(Na) is used as an active shield detector to suppress the background of NaI(Tl) and also serves as an all-sky gamma-ray burst monitor covering 0.2--3\,MeV. In this paper, we review the in-orbit performance of HE in the first 5 years since \textit{Insight}-HXMT was launched on June 15, 2017. Methods: The major performances we concern include the gain and energy resolution of NaI(Tl) and CsI(Na) detectors, the performance of pulse-shape-discriminator (PSD) and system dead-time. In this work, we investigate these performances mainly using the data of blank-sky observations and the data when the telescope in earth occultation. Results: The overall performance of HE/NaI(Tl) is very stable in the first 5 years, whereas the gain of HE/CsI(Na) shows a continuously increasing trend and should be calibrated regularly. Conclusion: In general, HE is still in good health and well-calibrated status after five-year's operation. The in-orbit performance of HE has no significant deviation from expectation. HE is expected to be in operation healthily for another several years of extended mission life.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


